Approximation Schemes for Many-Objective Query Optimization

The goal of multi-objective query optimization (MOQO) is to find query plans that realize a good compromise between conflicting objectives such as minimizing execution time and minimizing monetary fees in a Cloud scenario. A previously proposed exhaustive MOQO algorithm needs hours to optimize even simple TPC-H queries. This is why we propose several approximation schemes for MOQO that generate guaranteed near-optimal plans in seconds where exhaustive optimization takes hours. We integrated all MOQO algorithms into the Postgres optimizer and present experimental results for TPC-H queries; we extended the Postgres cost model and optimize for up to nine conflicting objectives in our experiments. The proposed algorithms are based on a formal analysis of typical cost functions that occur in the context of MOQO. We identify properties that hold for a broad range of objectives and can be exploited for the design of future MOQO algorithms.

==> Paper/sections/MOQOtemplate.tex <==
\section{Algorithmic Template for MOQO}
\label{templateSec}

We present an algorithmic template for MOQO. All algorithms that are presented and discussed in this paper (\AG{}, \AWM{}, \ABM{}) can be represented as instances of this template. Our template contains several placeholders, leaving details such as formulas and conditions open. We will describe the algorithms in Section~\ref{optimalEvalSec}, \ref{wMOQOsec}, and \ref{bMOQOsec} concisely by specifying concrete formulas and conditions for those placeholders. 

\begin{algorithm}[h!]
\input{../algorithms/Paper/templateMain1.tex}
\caption{Template for MOQO}
\label{templateMainAlg}
\end{algorithm}

Algorithm~\ref{templateMainAlg} shows pseudo-code of the main function of our algorithmic template. $\mathbf{X}_k$ marks the $k$-th placeholder in the code. Function {\tt MOQO} takes a MOQO problem and a precision $\alpha_U$ as input. Depending on the substitutions for $\mathbf{X}_1$ and $\mathbf{X}_2$, it either returns an optimal or an $\alpha_U$-approximate solution. The function is iterative. We calculate an internal approximation precision $\alpha_i$ in every iteration. We represent the formula for calculating $\alpha_i$ as placeholder $\mathbf{X}_1$ since it is algorithm-specific. We invoke function {\tt ParetoPlans} to calculate a set of plans for $Q$. {\tt ParetoPlans} returns either a Pareto plan set or an $\alpha_i^{|Q|-1}$-approximate Pareto set (depending on how the placeholders in {\tt ParetoPlans} are substituted). We discuss the pseudo-code of {\tt ParetoPlans} later. We select the optimal plan $p_{opt}$ out of the set returned by {\tt ParetoPlans}. The algorithm-specific termination condition of the main loop (placeholder $\mathbf{X}_2$) checks whether the cost of $p_{opt}$ is sufficiently close to the optimum. We return $p_{opt}$ in this case. Otherwise, we iterate and refine the internal precision which causes {\tt ParetoPlans} to return more plans. 

\begin{algorithm}[h!]
\input{../algorithms/Paper/ParetoApproximationTemplate1.tex}
\caption{Template for Calculating Pareto Plans}
\label{paretoSetTemplate}
\end{algorithm}

Algorithm~\ref{paretoSetTemplate} shows pseudo-code of function {\tt ParetoPlans}. Given query $Q$ and precision $\alpha_i$ as inputs, the function returns either a Pareto plan set or an $\alpha_i^{|Q|-1}$-approximate Pareto plan set (depending on the substitution for placeholder $\mathbf{X}_3$). The function uses dynamic programming: We calculate (approximate) Pareto sets for a non-singleton table set out of (approximate) Pareto sets of the subsets. For singleton table sets, we return all available access paths. For non-singleton table sets, we decompose set $Q$ in all possible ways (so we consider bushy plans) and calculate plans for joining the subsets by recursive invocations. For every decomposition into two subsets $q_1$, $q_2$, we combine all recursively generated plans for $q_1$ and $q_2$ into plans for $S$, using all available join operators $j\in\mathbb{J}$. We insert a new plan $p_N$ into plan set $\mathcal{P}^Q$ only if it passes a test that differs among the different algorithms. The condition for inserting the new plan is the third placeholder. If the new plan is inserted, we delete all plans in $\mathcal{P}^S$ that are dominated by the new plan. We do not need to keep dominated plans in the set, since the dominant plans would be preferable in each case. Pruning out as many plans as possible increases efficiency since less plans have to be treated in future processing steps. In order to keep our pseudo-code simple, we do not take into account interesting orders~\cite{selinger1979access}. Extending the algorithm is straight-forward and our implementation takes interesting orders into account. 

We discuss two fundamental design choices of our algorithmic template. First, our template uses dynamic programming: we generate plans bottom-up, calculating near-optimal plans for joining a set of tables out of near-optimal plans for joining its subsets. We adopt this approach because it has been extremely successful for cost-based SOQO (it is used by the seminal Selinger algorithm~\cite{Selinger1979} and its many derivatives). Second, our algorithmic template is iterative, refining the approximation of the Pareto set step by step. There are problem variants in which it is not clear a-priori, which internal precision $\alpha_i$ must be chosen to guarantee that an $\alpha_U$-optimal solution is generated. Even if such an $\alpha_i$ can be calculated, it is likely that we find an $\alpha_U$-optimal solution even with a more coarse-grained precision and we have conditions that allow to recognize such a solution. An non-iterative approach would miss the occasion to benefit from this fact and the complexity of the Pareto set approximation quickly increases once precision is refined. The only potential drawback of an iterative approach is redundant work over different iterations. We will present precision refinement schemes that guarantee that the amount of redundant work is negligible. 


==> algorithms/Paper/ParetoApproximationTemplate1.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\vspace{0.5cm}
\begin{algorithmic}[1]
\State \Comment{Depending on substitutions for $\mathbf{X}_3$, returns }
\State \Comment{either a Pareto set for query $Q$ or an}
\State \Comment{$\alpha_i^{|Q|-1}$-approximate Pareto set}
\Function{ParetoPlans}{$Q,\alpha_i$}
\State \Comment{Calculate plans for singleton sets}
\ForAll{$q\in Q$} 
\State $\mathcal{P}^{q}\leftarrow$ Optimal access paths to $q$
\EndFor
\State \Comment{Consider table sets of increasing cardinality}
\ForAll{$k\in2..|Q|$}
\ForAll{$q\subseteq Q:|q|=k$}
\State $\mathcal{P}^{q}\leftarrow\emptyset$
\State \Comment{For all possible splits of set $q$}
\ForAll{$q_{1},q_{2}\subset q:q_{1}\dot{\cup}q_{2}=q$}
\State \Comment{For all subplans and operators}
\ForAll{$p_{1}\in\mathcal{P}^{q_1},p_{2}\in\mathcal{P}^{q_2},j\in\mathbb{J}$}
\State \Comment{Construct new plan out of subplans}
\State $p_N\leftarrow\mathrm{Combine}(j,p_{1},p_{2})$
\State \Comment{Check whether new plan useful}
\If{$\mathbf{X}_3$}
\State \Comment{Delete dominated plans}
\State $\mathcal{P}^q\leftarrow\{p\in\mathcal{P}^q|\neg(\mathbf{c}(p_N)\preceq\mathbf{c}(p))\}$
\State \Comment{Insert new plan}
\State $\mathcal{P}^q\leftarrow\mathcal{P}^q\cup\{p_N\}$
\EndIf
\EndFor
\EndFor
\EndFor
\EndFor
\State \Return{$\mathcal{P}^Q$}
\EndFunction
\end{algorithmic}


==> algorithms/Paper/bMOQOadd.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Move plan $p$ for joining set $S$ from pool $\mathcal{P}^S_{pool}$ to}
\State \Comment{current approximation set $\mathcal{P}^S$, update critical}
\State \Comment{precision of table set ($\alpha_C(S)$) and of plans in pool}
\Procedure{AddFromPool}{$p,S$}
\State \Comment{Delete plan from pool}
\State $\mathcal{P}^S_{pool}\leftarrow\mathcal{P}^S_{pool}\setminus\{p\}$
\State \Comment{Delete dominated approximation plans}
\State $\mathcal{P}^S\leftarrow\mathcal{P}^S\setminus\{\widetilde{p}\in\mathcal{P}^S|p\preceq\widetilde{p}\}$
\State \Comment{Add plan to approximation plans}
\State $\mathcal{P}^S\leftarrow\mathcal{P}^S\cup\{p\}$
\State \Comment{Recalculate critical precision of pooled plans}
\ForAll{$\widetilde{p}\in\mathcal{P}^S_{pool}:$ $\alpha_C(\widetilde{p})$ might have changed}
\State $\alpha_C(\widetilde{p})\leftarrow\min(\alpha_C(\widetilde{p}),prec(p,\widetilde{p}))$
\EndFor
\EndProcedure
\end{algorithmic}


==> algorithms/Paper/bMOQOmain2.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Update table set $S$ by refining the PPSA to}
\State \Comment{precision $\alpha$, calculate critical precision $\alpha_C(S)$}
\Procedure{UpdateTS}{$S,\alpha$}
\State \Comment{Update table subsets and propagate changes}
\ForAll{$sub\subset S:sub\neq\emptyset,\alpha_{C}(sub)>\alpha$}
\State UpdateTS($sub,\alpha$)
\State Propagate($sub,S$)
\EndFor
\State \Comment{For all plans in $\mathcal{P}^S_{pool}$ that cannot be approximated}
\ForAll{$p\in\mathcal{P}^{S}_{pool}:\nexists\widetilde{p}\in\mathcal{P}^S:\widetilde{p}\preceq_{\alpha}p$}
\State \Comment{Delete plan from pool}
\State $\mathcal{P}^S_{pool}\leftarrow\mathcal{P}^S_{pool}\setminus\{p\}$
\State \Comment{Add new plan and delete dominated plans}
\State $\mathcal{P}^S\leftarrow(\mathcal{P}^S\setminus\{\widetilde{p}\in\mathcal{P}^S|p\preceq\widetilde{p}\})\cup\{p\}$
%\State AddFromPool($p,S$) \Comment{add to $\mathcal{P}^S$}
\EndFor
\State \Comment{Calculate critical precision of table set}
\State $\alpha_C(S)\leftarrow\max($
\Statex \hspace{\algorithmicindent}\hspace{\algorithmicindent}$\{\min[\widetilde{p}\in\mathcal{P}^S]prec(\widetilde{p},p)|p\in\mathcal{P}^S_{pool}\}\cup$
\Statex \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}$\{\alpha_C(sub)|sub\subset S\}\cup\{-\infty\})$
\EndProcedure
\end{algorithmic}


==> algorithms/Paper/bMOQOprop.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Propagate changes in PPSA of table set $sub$}
\State \Comment{to $S\supset sub$ by adding/deleting plans in $P^S$ and $P^S_{pool}$}
\Procedure{Propagate}{$sub,S$}
\State $\Delta^+\leftarrow$ Plans added to $\mathcal{P}^{sub}$ in this iteration
\State $\Delta^-\leftarrow$ Plans deleted from $\mathcal{P}^{sub}$ in this iteration
\State \Comment{Delete plans constructed from deleted sub-plans}
\ForAll{$p^-\in\Delta^-$}
\ForAll{$p\in\mathcal{P}^S\cup\mathcal{P}^S_{pool}:$ $p$ uses $p^-$}
\State $\mathcal{P}^S\leftarrow\mathcal{P}^S\setminus\{p\};\mathcal{P}^S_{pool}\leftarrow\mathcal{P}^S_{pool}\setminus\{p\}$
\EndFor
\EndFor
\State \Comment{Construct plans from added sub-plans}
\ForAll{$p_1\in\Delta^+,p_2\in\mathcal{P}^{S\setminus sub}$}
\State $p\leftarrow\mathrm{Combine}(p_1,p_2)$
\State \Comment{If new plan not dominated and respects $\alpha_i\mathbf{B}$}
\If{$\mathbf{c}(p)\preceq\alpha_i\mathbf{B}\wedge\nexists\widetilde{p}\in\mathcal{P}^S\cup\mathcal{P}^S_{pool}:\widetilde{p}\preceq p$}
\State \Comment{Add new plan and delete dominated plans}
\State $\mathcal{P}^S_{pool}\leftarrow(\mathcal{P}^S_{pool}\setminus\{\widetilde{p}\in\mathcal{P}^S_{pool}|p\preceq\widetilde{p}\})\cup\{p\}$
%\State \Comment{Calculate critical precision for new plan}
%\State $\alpha_C(p)\leftarrow\min[\widetilde{p}\in\mathcal{P}^S]prec(p,\widetilde{p})$
\EndIf
\EndFor
\EndProcedure
\end{algorithmic}


==> algorithms/Paper/wMOQO2.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Approximate set of Pareto-optimal plans}
\State \Comment{for table set $S$ using precision $\alpha$}
\Procedure{ApproximateTS}{$S,\alpha$}
\State \Comment{Calculate plans for table subsets}
\ForAll{$sub\subset S:sub=\emptyset,\mathcal{P}^{S}=\emptyset$} 
\State ApproximateTS($sub,\alpha$)
\EndFor
\State \Comment{Whether $S$ is single table}
\If{$|S|=1$}
\State $\mathcal{P}^{S}\leftarrow$ Optimal access paths to $S$
\Else
\State $\mathcal{P}^{S}\leftarrow\emptyset$
\State \Comment{For all possible splits of set $S$}
\ForAll{$s_{1},s_{2}\subset S:s_{1}\dot{\cup}s_{2}=S$}
\State \Comment{For all combinations of subplans}
\ForAll{$p_{1}\in\mathcal{P}^{s1},p_{2}\in\mathcal{P}^{s2}$}
\State \Comment{Construct new plan out of subplans}
\State $p\leftarrow\mathrm{Combine}(p_{1},p_{2})$
\State \Comment{If new plan cannot be approximated}
\If{$\neg\exists\widetilde{p}\in\mathcal{P}^{S}:\widetilde{p}\preceq_{\alpha} p$} 
\State $\mathcal{P}^{S}\leftarrow(\mathcal{P}^{S}\setminus\{\widetilde{p}\in\mathcal{P}^{S}|p\preceq\widetilde{p}\})\cup\{p\}$
\EndIf
\EndFor
\EndFor
\EndIf
\EndProcedure
\end{algorithmic}


==> algorithms/bMOQOclean.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Remove plans from $\mathcal{P}_{cur}(S)$ that use subplans for $sub\subseteq S$ that were deleted}
\Function{CleanUp}{$S,sub$}
\ForAll{$p\in\mathcal{P}_{del}^{sub}$}
\State $\mathcal{P}_{cur}^{S}\leftarrow\{\widetilde{p}\in\mathcal{P}_{cur}^{S}|\text{$\widetilde{p}$ does not use $p$ as subplan}\}$
\State $\mathcal{P}_{PB}^{S}\leftarrow\{\widetilde{p}\in\mathcal{P}_{PB}^{S}|\text{$\widetilde{p}$ does not use $p$ as subplan}\}$
\EndFor
\EndFunction
\end{algorithmic}


==> algorithms/bMOQOmain.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Updates a table set $S$ by refining the approximation and calculating $\alpha_{C}$}
\Function{UpdateTS}{$S,\alpha$}
\ForAll{$sub\in\mathrm{Split}(S):\alpha_{C}(sub)\geq\alpha$} \Comment{Update subsets, propagate deletes}
\State UpdateTS($sub,\alpha$); CleanUp($S,sub$)
\EndFor
\State $\mathcal{P}^{S}_{next}\leftarrow\mathrm{NextPlans}(S)$ \Comment{Determine new plans to consider in this iteration}
\State \Comment{Treat every new plan and update plan sets accordingly}
\ForAll{$p\in\mathcal{P}^{S}_{next}$}
\If{$\nexists\widetilde{p}\in\mathcal{P}^{S}_{cur}\cup\mathcal{P}^{S}_{PB}:\widetilde{p}\preceq p$} \Comment{If new plan is not dominated}
\If{$\exists\widetilde{p}\in\mathcal{P}^{S}_{cur}:\widetilde{p}\preceq_{\alpha}p$} \Comment{If new plan can be approximated}
\State $\mathcal{P}^{S}_{PB}\leftarrow(\mathcal{P}^{S}_{PB}\setminus\{\widetilde{p}\in\mathcal{P}^{S}_{PB}|p\preceq\widetilde{p}\})\cup\{p\}$
\Else \Comment{If new plan cannot be approximated}
\State $\mathcal{P}^{S}_{cur}\leftarrow(\mathcal{P}^{S}_{cur}\setminus\{\widetilde{p}\in\mathcal{P}^{S}_{cur}|p\preceq\widetilde{p}\})\cup\{p\}$
\EndIf
\EndIf
\EndFor
\State $\mathcal{P}^{S}_{add}\leftarrow$ Plans added to $\mathcal{P}_{cur}^{S}$ in this iteration
\State $\mathcal{P}^{S}_{del}\leftarrow$ Plans deleted from $\mathcal{P}_{cur}^{S}$ in this iteration
\State $\alpha_{C}(S)\leftarrow\mathrm{CalculateCriticalPrecision}(S)$ \Comment{Calculate critical precision for $S$}
\EndFunction
\end{algorithmic}


==> algorithms/bMOQOnext.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Calculate sets of plans that to consider for table set $S$ during this iteration}
\Function{NextPlans}{$S,\alpha$}
\State $\mathcal{P}_{next}^{S}\leftarrow\emptyset$
\State \Comment{Recheck all plans that could be approximated before whether still the case}
\ForAll{$p\in\mathcal{P}^{S}_{PB}$}
\If{$\nexists\widetilde{p}\in\mathcal{P}_{cur}^{S}:\widetilde{p}\preceq_{\alpha}p$}
\State $\mathcal{P}^{S}_{next}\leftarrow\mathcal{P}^{S}_{next}\cup\{p\}$
\EndIf
\EndFor
\State \Comment{Combine plans that include freshly added subplans for subsets of $S$}
\ForAll{$sub\in\mathrm{Split}(S)$} \Comment{For all possible splits of $S$}
\ForAll{$p_{1}\in\mathcal{P}^{sub}_{add},p_{2}\in\mathcal{P}_{cur}^{S\setminus sub},op\in JoinOps$}
\State $\mathcal{P}_{next}^{S}\leftarrow\mathcal{P}_{next}^{S}\cup\{\mathrm{Combine}(p_{1},p_{2},op)\}$
\EndFor
\EndFor
\State \Return{$\mathcal{P}_{next}^{S}$}
\EndFunction
\end{algorithmic}


==> algorithms/bMOQOprecision.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Calculates critical precision $\alpha_{C}(S)$ for a table set $S$}
\Function{CalculateCriticalPrecision}{$S$}
\State $\alpha_{C}(S)\leftarrow1$
\State \Comment{Determine maximum $\alpha$ for which plans in $\mathcal{P}_{PB}^{S}$ become interesting}
\ForAll{$p\in\mathcal{P}_{PB}^{S}$}
\State $\alpha_{C}(p)\leftarrow\infty$
\ForAll{$\widetilde{p}\in\mathcal{P}_{cur}^{S}$} \Comment{Search for best approximation plan}
\State $\alpha_{C}^{p,\widetilde{p}}\leftarrow$ minimum $\alpha$ s.t. $\widetilde{p}\preceq_{\alpha}p$
\State $\alpha_{C}(p)\leftarrow\min(\alpha_{C}(p),\alpha_{C}^{p,\widetilde{p}})$
\EndFor
\State $\alpha_{C}(S)\leftarrow\max(\alpha_{C}(S),\alpha_{C}(p))$
\EndFor
\State \Comment{Take into account $\alpha_{C}$ of subsets since changes might propagate to $S$}
\State $\alpha_{C}(S)\leftarrow\max(\{\alpha_{C}(S)\}\cup\{\alpha_{C}(sub)|sub\in\mathrm{Split}(S)\})$
\State \Comment{Return critical precision for $S$}
\State \Return{$\alpha_{C}(S)$}
\EndFunction
\end{algorithmic}


==> algorithms/wMOQO.tex <==
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{algorithmic}[1]
\State \Comment{Approximate set of Pareto-optimal plans for table set $S$ using precision $\alpha$}
\Procedure{ApproximateTS}{$S,\alpha$}
\ForAll{$sub\in\mathrm{Split}(S)$} \Comment{Calculate plans for subsets}
\State ApproximateTS($sub,\alpha$)
\EndFor
\State \Comment{Consider every plan that can be constructed from plans for subsets}
\State $\mathcal{P}^{S}\leftarrow\emptyset$
\ForAll{$p:p=\mathrm{Combine}(p_{1},p_{2}),p_{1}\in\mathcal{P}^{s1},p_{2}\in\mathcal{P}^{s2},s1\cup s2=S$}
%\If{$\nexists\widetilde{p}\in\mathcal{P}^{S}:\widetilde{p}\preceq_{\alpha} p$} \Comment{If new plan cannot be approximated}
\State $\mathcal{P}^{S}\leftarrow(\mathcal{P}^{S}\setminus\{\widetilde{p}\in\mathcal{P}^{S}|p\preceq\widetilde{p}\})\cup\{p\}$
%\EndIf
\EndFor
\EndProcedure
\end{algorithmic}


==> figures/algorithmOutlines/bMOQOoutline1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
  \pgfsetlinewidth{1bp}
%%
\pgfsetcolor{black}
  % Edge: check -> select
  \draw [->] (125.91bp,79.934bp) .. controls (125.91bp,73.086bp) and (125.91bp,64.167bp)  .. (125.91bp,46.241bp);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (136.1bp,63bp) node {Yes};
  % Edge: approximation -> check
  \draw [->] (141.67bp,121.64bp) .. controls (140.21bp,119bp) and (138.63bp,116.12bp)  .. (132.1bp,104.25bp);
  % Edge: precision -> approximation
  \draw [->] (121.42bp,163.64bp) .. controls (124.25bp,160.58bp) and (127.4bp,157.18bp)  .. (137.51bp,146.25bp);
  % Edge: input -> precision
  \draw [->] (110.91bp,205.9bp) .. controls (110.91bp,203.7bp) and (110.91bp,201.08bp)  .. (110.91bp,188.25bp);
  % Edge: check -> precision
  \draw [->] (25.912bp,92bp) .. controls (-7.8347bp,92bp) and (-7.0592bp,160.39bp)  .. (30.912bp,176bp);
  \draw (25.825bp,134bp) node {Not sure};
  % Edge: select -> output
  \draw [->] (125.91bp,31.929bp) .. controls (125.91bp,29.652bp) and (125.91bp,26.943bp)  .. (125.91bp,14.062bp);
  % Node: precision
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (190bp,188bp) -- (32bp,188bp) -- (32bp,164bp) -- (190bp,164bp) -- cycle;
  \draw (110.91bp,176bp) node {\parbox{2.2in}{\centering Select precision $\alpha_i$ for next iteration $i$\\(see Section~\ref{selectPrecisionSub}}};
\end{scope}
  % Node: approximation
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (227bp,146bp) -- (69bp,146bp) -- (69bp,122bp) -- (227bp,122bp) -- cycle;
  \draw (147.91bp,134bp) node {\parbox{2.2in}{\centering Approximate Pareto set with prec. $\alpha_i$\\(see Section~\ref{incrementalApproximationSub}, Algorithm~\ref{bMOQOalg})}};
\end{scope}
  % Node: output
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (125.91bp,7bp) node {Near-optimal plan or no solution};
\end{scope}
  % Node: input
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (110.91bp,213bp) node {BMOQO problem $I=\langle Q,\mathbf{W},\mathbf{B},\alpha_U\rangle$};
\end{scope}
  % Node: check
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (217bp,104bp) .. controls (217bp,104bp) and (35bp,104bp)  .. (35bp,104bp) .. controls (31bp,104bp) and (27bp,100bp)  .. (27bp,96bp) .. controls (27bp,96bp) and (27bp,88bp)  .. (27bp,88bp) .. controls (27bp,84bp) and (31bp,80bp)  .. (35bp,80bp) .. controls (35bp,80bp) and (217bp,80bp)  .. (217bp,80bp) .. controls (221bp,80bp) and (225bp,84bp)  .. (225bp,88bp) .. controls (225bp,88bp) and (225bp,96bp)  .. (225bp,96bp) .. controls (225bp,100bp) and (221bp,104bp)  .. (217bp,104bp);
  \draw (125.91bp,92bp) node {\parbox{2.75in}{\centering Retrieved near-optimal plan?\\(see Section~\ref{stoppingConditionSub})}};
\end{scope}
  % Node: select
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (225bp,46bp) -- (27bp,46bp) -- (27bp,32bp) -- (225bp,32bp) -- cycle;
  \draw (125.91bp,39bp) node {Select best plan respecting bounds $\mathbf{B}$};
\end{scope}
%
\end{tikzpicture}


==> figures/algorithmOutlines/wMOQOoutline1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
  \pgfsetlinewidth{1bp}
%%
\pgfsetcolor{black}
  % Edge: input -> precision
  \draw [->] (108bp,137.93bp) .. controls (108bp,135.65bp) and (108bp,132.94bp)  .. (108bp,120.06bp);
  % Edge: approximation -> selection
  \draw [->] (108bp,63.926bp) .. controls (108bp,61.425bp) and (108bp,58.721bp)  .. (108bp,46.017bp);
  % Edge: selection -> output
  \draw [->] (108bp,31.929bp) .. controls (108bp,29.652bp) and (108bp,26.943bp)  .. (108bp,14.062bp);
  % Edge: precision -> approximation
  \draw [->] (108bp,105.9bp) .. controls (108bp,103.7bp) and (108bp,101.08bp)  .. (108bp,88.255bp);
  % Node: approximation
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (216bp,88bp) -- (0bp,88bp) -- (0bp,64bp) -- (216bp,64bp) -- cycle;
  \draw (108bp,76bp) node {\parbox{3in}{\centering Approximate Pareto set with precision $\alpha$\\(see Section~\ref{wApproximationSub}, Algorithm~\ref{wMOQOalg})}};
\end{scope}
  % Node: input
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (108bp,145bp) node {WMOQO problem $I=\langle Q,\mathbf{W},\alpha_U\rangle$};
\end{scope}
  % Node: selection
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (216bp,46bp) -- (0bp,46bp) -- (0bp,32bp) -- (216bp,32bp) -- cycle;
  \draw (108bp,39bp) node {Select optimal plan out of approximated Pareto set};
\end{scope}
  % Node: precision
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (216bp,120bp) -- (0bp,120bp) -- (0bp,106bp) -- (216bp,106bp) -- cycle;
  \draw (108bp,113bp) node {Select internal precision $\alpha=\sqrt[n]{\alpha_U}$};
\end{scope}
  % Node: output
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (108bp,7bp) node {Near-optimal query plan};
\end{scope}
%
\end{tikzpicture}


==> figures/diagrams/realParetoSurfaceCoarse.tex <==
\begin{tikzpicture}
\begin{axis}[
xlabel=Time,
ylabel=Tuple Loss,
ylabel near ticks,
xlabel near ticks,
axis x line=bottom,
axis y line=left,
width=4cm,height=3cm]
    \addplot[only marks,mark=x,thick] table {figures/diagrams/time_loss_c3_24sec.dat};
\end{axis}
\end{tikzpicture}

==> figures/diagrams/realParetoSurfaceFine.tex <==
\begin{tikzpicture}
\begin{axis}[
xlabel=Time,
ylabel=Tuple Loss,
ylabel near ticks,
xlabel near ticks,
axis x line=bottom,
axis y line=left,
width=4cm, height=3cm]
    \addplot[only marks,mark=x,thick] table {figures/diagrams/time_loss_c1_5_235sec.dat};
\end{axis}
\end{tikzpicture}
